Capek 0.5: An Execution-Centric Vision-Language Model for Embodied Intelligence

Vision-language models are increasingly serving as the reasoning core of embodied agents. Robot execution is inherently iterative: each action reshapes the scene and physical state, continually renewing what must be perceived, reasoned about, and verified. Meeting these demands requires complementary capabilities that differ in supervision signals, prediction formats, and verification criteria. Existing approaches typically develop these capabilities against isolated, task-specific objectives, leaving open how they should be organized and integrated around execution as a whole. We present Capek 0.5, an embodied vision-language model built around an execution-centric capability taxonomy. Rather than organizing training by datasets or tasks, the taxonomy groups embodied capabilities according to their functional roles throughout execution and comprises four capability families: Spatial Reasoning, Temporal Understanding, Action Guidance, and State Verification. Each capability is first acquired by a dedicated specialist through reinforcement learning with verifiable rewards from a shared backbone, and the specialists are then consolidated into a single inference-time model through weight-space merging followed by routed policy-space distillation. We instantiate Capek 0.5 at the 2B and 35B-A3B scales and evaluate it from three complementary perspectives: comprehensive benchmark suites including Capek-StateBench, a new benchmark for state verification; a controlled study of capability retention from specialists to the unified model; and closed-loop evaluation in simulated embodied environments. Capek 0.5 improves the large majority of matched benchmark rows over its initialization, retains all four specialized capabilities in one checkpoint with quantified losses, and transfers to closed-loop embodied task execution.

==> main/contributions.tex <==
\section*{Contributions and Acknowledgments}
\label{sec:contributions}
\addcontentsline{toc}{section}{Contributions and Acknowledgments}

% TODO(owner): fill the real contributor roster before public release. The grouping below follows
% the expert-production, integration, and evaluation structure of the report.

\paragraph{Data.}
% TODO(owner): names — Guidance point/trajectory, Temporal, Spatial, State, and Task Progress
% data cards, filtering pipelines, and diagnostic examples.
\xvista Team.

\paragraph{Training and integration.}
% TODO(owner): names — SFT/CoT, verifier-driven RL/GRPO, OPD/MOPD integration, and merge/checkpoint selection.
\xvista Team.

\paragraph{Evaluation and infrastructure.}
  % TODO(owner): names — DeepInsight evaluation harness, benchmark curation, State/Task Progress evaluation, and VIGIL runs.
\xvista Team.

\paragraph{Acknowledgments.}
% TODO(owner): acknowledge compute, internal reviewers, and the teams behind the DeepInsight and VIGIL tooling.
We thank the teams who supported evaluation infrastructure and internal review of this report.

